Statistical Reachability Analysis of Stochastic Cyber-Physical Systems under Distribution Shift

Reachability analysis is a popular method to give safety guarantees for stochastic cyber-physical systems (SCPSs) that takes in a symbolic description of the system dynamics and uses set-propagation methods to compute an overapproximation of the set of reachable states over a bounded time horizon. In this paper, we investigate the problem of performing reachability analysis for an SCPS that does not have a symbolic description of the dynamics, but instead is described using a digital twin model that can be simulated to generate system trajectories. An important challenge is that the simulator implicitly models a probability distribution over the set of trajectories of the SCPS; however, it is typical to have a sim2real gap, i.e., the actual distribution of the trajectories in a deployment setting may be shifted from the distribution assumed by the simulator. We thus propose a statistical reachability analysis technique that, given a user-provided threshold $1-\epsilon$, provides a set that guarantees that any reachable state during deployment lies in this set with probability not smaller than this threshold. Our method is based on three main steps: (1) learning a deterministic surrogate model from sampled trajectories, (2) conducting reachability analysis over the surrogate model, and (3) employing {\em robust conformal inference} using an additional set of sampled trajectories to quantify the surrogate model's distribution shift with respect to the deployed SCPS. To counter conservatism in reachable sets, we propose a novel method to train surrogate models that minimizes a quantile loss term (instead of the usual mean squared loss), and a new method that provides tighter guarantees using conformal inference using a normalized surrogate error. We demonstrate the effectiveness of our technique on various case studies.

==> sections/revision.tex <==
\section{Revision letter}
We thank the reviewers for their time and  valuable comments. Given the \textbf{3 page limit of this revision letter}, we first address the
high-level comments raised by the meta-reviews, and then address comments raised
by individual reviews.

\mypara{Paper is dense} We are constrained by the 12 page limit, but have
made several efforts to improve readability of the paper in the revision. If the
paper is accepted, we will also provide an extended version of the paper on
arXiv which will include detailed explanations for the technical parts and
 experiments.

\mypara{Surrogate Models, Choice of NN-based surrogates} We have added a formal
definition of a surrogate model and a section to more formally describe the
properties of the surrogate model. We can work with arbitrary surrogate models
such as Gaussian Processes and other data-driven models (obtained by system
identification). We choose DNN-based surrogates for two main reasons: (1) DNNs
have computational advantages in learning (data efficiency, using stochastic
gradient descent and leveraging GPUs for training), and (2) exact and
approximate set propagation techniques for DNNs perform comparably to
state-of-the-art reachability analysis for dynamical system models. Finally,
several popular methods in  model-based RL and neural MPC use DNN-based
surrogates \cite{nagabandi2018neural,salzmann2023real,chua2018deep}.

\mypara{Restriction to ReLU activation function} Our proposed method applies
broadly to DNNs with arbitrary activation functions. However, in practice to
perform reachability analysis, we rely on efficient algorithms for ReLU
activation functions, which is why that in this paper, we choose ReLUs. In the
future we will investigate tools such as alpha-beta-Crown to handle other kinds
of nonlinear activations. 

\mypara{Training and Validity of Surrogate Models} The reviewers rightly point
to the tendency of DNNs to overfit to data; a limitation shared by the MSE-based
training approaches such as in \cite{hashemi2023data}. A DNN-surrogate that has
low prediction error over most data points but high error for a few may still
have low MSE error. A quantile-based loss avoids this problem as it improves the
{\em distribution of residual errors}. This can in many cases prevent
overfitting. Another mechanism that indirectly reduces overfitting is
Lipschitz-constant-constrained training. This prevents large deviations in the
output of the DNN for proximal inputs; a common phenomenon when an NN overfits
to the data.  The Lipschitz-constant-constrained training also uses tricks such
as weight regularization --  a common way to reduce overfitting in machine
learning.

\mypara{Benefits of quantile minimization comparing to MSE} The MSE loss
function is a standard choice in NN training and could also be used in
conjunction with our proposed method. However, as our method aims to construct
reachable sets that cover $\bar{\delta}$ percent of the trajectories, the
$\bar{\delta}$-quantile based loss function is a more natural choice that
results in smaller errors as we empirically show in the paper. On the other
hand, the MSE loss function only minimizes the expected loss and may thus result
in large errors in the tail of the distribution, ultimately resulting in
conservative reachable sets. 

\mypara{Quality of Surrogate Models} Conformal inference is a technique to
obtain confidence intervals on predictive models in machine learning. We
extensively employ CI to validate our surrogate models as seen in the paper. As
we are interested in handling real-world systems, it is impossible to obtain any
formal guarantees except for those obtained through statistical techniques and
like conformal prediction. While it is possible to get deterministic guarantees
on a surrogate model (for example an ODE-based model), these models may still
have sim2real gap. We explicitly address this through our use of robust
conformal inference.

\mypara{Connections to Existing Literature} As suggested by R2, we have moved
 related work right after the introduction. We have also given more details
about  connections with  related work.





%We can also add the loss function $\loss_2$ is nothing but an approximation for $R^{*}_{\delta,\tau}(\frac{1}{\alpha_1}+...+\frac{1}{\alpha_{n\horizon}})$ which is exactly the surface area of inflating zonotope. 

% Based on the comments of the majority of reviewers, we have decided to do not claim the methodology is restricted to a ReLU NN. We removed it from the body of paper, but we included a remark in the experiment section that we suggest using ReLU NN surrogate models. This suggestion is motivated by the fact that, the recent achievement in the literature (NNV toolbox) has provided fantastic results for NN reachability which is limited to ReLU activation function, and We found this advantage sufficient to decide to restrict our toolbox only to ReLU neural networks. In case we utilize other activation functions, we expect conservative results, as the surrogate reachability can not be handled very well.   

% Yes, we have restricted our toolbox to ReLU activation function. This choice is motivated by the fact that, the recent achievements in the literature (NNV toolbox) has provided fantastic results for NN reachability which is limited to ReLU activation function. We found this advantage sufficient to decide to restrict our toolbox only to ReLU neural networks. This is why the ReLU NN is applied systematically in the paper. In the revised version of the document, it is now apparent that the technique is solely proposed for ReLU neural networks and in case we utilize other activations then the probabilistic reachable set becomes conservative. While we can use all the 


\mypara{\bf Evaluation parameters}: In the experiments, we have added more explanation to the column titles in the tables and
added a small remark about how various parameters for  were chosen. 



We note that some of the individual reviewer concerns addressed above
are not repeated in the responses below.

%  (despite being dense) and interesting; the evaluation on a
% quadrotor was also appreciated. However, the reviewers had several important
% concerns, especially regarding the surrogate model training, that need to be
% addressed in the second round revision. For example, there were questions about
% how the work addresses known problems associated with NN models (such as
% over-fitting, optimal selection of model architectures, etc.), about the quality
% of the surrogate model and the reliability of the results. The paper currently
% also lacks proper definitions, formal characterizations of the surrogate model's
% properties, and a validation of the model itself. The connections and
% enhancement to existing literature should also be made much clearer. There were
% also questions regarding the choice and explanation of the parameters used in
% the evaluation. The authors should go through the in dividual reviews carefully
% and address the concerns raised therein.
% \begin{itemize}[wide,labelwidth!=labelinde]
% 
% paper well-writtennt=0pt

% (despite being dense) and interesting; the evaluation on a
% quadrotor was also appreciated. However, the reviewers had several important
% concerns, especially regarding the surrogate model training, that need to be
% addressed in the second round revision. For example, there were questions about
% how the work addresses known problems associated with NN models (such as
% over-fitting, optimal selection of model architectures, etc.), about the quality
% of the surrogate model and the reliability of the results. The paper currently
% also lacks proper definitions, formal characterizations of the surrogate model's
% properties, and a validation of the model itself. The connections and
% enhancement to existing literature should also be made much clearer. There were
% also questions regarding the choice and explanation of the parameters used in
% the evaluation. The authors should go through the individual reviews carefully
% and address the concerns raised therein.

\newcounter{myquestion}
\setcounter{myquestion}{0}
\newcommand{\question}[1]{\stepcounter{myquestion}\noindent \textbf{Q\themyquestion. } {\em #1} \\}
\newcommand{\answer}[1]{\noindent \textbf {A\themyquestion.} #1 \vspace{0.3em}}


\mypara{Reviewer 1}

\question{Is the method restricted to finite-horizon reachability?}
\answer{We remark that most set-propagation-based reachability analysis techniques studied in
the continuous and hybrid systems community are restricted to
finite time-horizons, e.g., see
\cite{chen2013flow,althoff2015introduction,huang2019reachnn,frehse2011spaceex,dutta2019sherlock,dryvr}.
Some early methods for reachability analysis do handle infinite horizon
properties if the reachable-set computation reaches a fixed point
\cite{frehse2011spaceex}. However, this is only theoretically possible for
contractive/Lyapunov-stable systems. Even for such systems, over-approximation
errors in set propagation make it difficult to obtain fixed points.  Given the
additional aspect of inflating the computed reach set with error analysis, it is
not clear to us how fixed-point based techniques would extend to
our setting. Other techniques such as those based on barrier certificates can
give infinite horizon guarantees, but require symbolic models of the
system.}

% \begin{itemize}[wide, labelwidth=!, labelindent=0pt,nosep]
%    \item Weakness 1:  We added a definition for surrogate model, and also we included a new section that describes the surrogate model's properties and the training algorithm.
%     \item Comment 1 (\textcolor{red}{Jyo takes care of this}): 

% Exactly, it may not scale to an infinite horizon. There are many approaches that seem to extend this method to an infinite horizon, but I will explain why all of them fail in practice. 1) One way is to include union bound which is discussed in comment "Experiment, comment 8" for Reviewer 2. But the union bound will be problematic for infinite horizon. 2) One other way is to train the model to receive a portion of the trajectory and predict the rest, in order to use this model repetitively. This fails because repeating the model results in the accumulation of errors over time and may lead to trivial bounds from surrogate reachability analysis. 2) Another approach is to train a single model that maps the initial state to a very long trajectory. This also does not scale because for a very long trajectory, the training process becomes prohibitively difficult, and the surrogate reachability becomes completely inefficient or highly conservative.   

\question{How is the Lipschitz constant restricted over the training process?}
\answer{The training algorithm penalizes the Lipschitz constant if it goes beyond a specified 
threshold. This is done using a regularization technique that is discussed in 
\cite{gouk2021regularisation} where the neural network training problem is a 
constrained optimization problem solved using projected stochastic gradient descent.}
    
% and we can not show it as an additive part to loss function. 
% We also need to make it clear that the Lipschitz constant is for the output of the NN (Trajectory). Finally, in this training process, this specific regularization part is considered to be separate from the proposed loss function and directly addresses the hidden layers of NN (i.e. the parameters $\theta$). For example, in this research, it does not affect $q, \alpha_j, j\in[n\horizon]$.  

% The main reason for the preference of quantile minimization over minimizing the mean (MSE) is its contribution to the reachability analysis. In other word, the inflating zonotope is generated based on the quantile and its surface area can be formulated as, $R^* \sum_{j=1}^{n\horizon} 1/\alpha_j$. Here $R^*$ is in fact the conformalized $\bar{\delta}$-quantile, for the residuals in training environment. Our ultimate goal in the training process is to minimize this surface area. $R^*$ is reachable only from KKT condition, which is expensive and inefficient, so we decided to approximate $R^*$ with the real $\bar{\delta}$-quantile. We assigned the trainable parameter $q$ for this purpose and introduced the loss $\loss_1$ to make it certain it serves as the $\bar{\delta}$-quantile. Next, we introduced $\loss_2$ to represent the surface of inflating zonotope. The training section was initially introduced at the end of the document, but we decided to move it to the beginning. This is exactly why we introduced $\loss_2$ as the average error over the trajectory. In case this provides ambiguity, we can move this section to the end again in camera ready submission and motivate it using the surface area of zonotope to make it more clear. By the way, in general, the quantile minimization is also more preferable to MSE. The quantile minimization focuses on the tail of the error's distribution, while the MSE only focuses on the expectation. In this case, the long tail may result in large quantile and provides us a conservative inflating zonotope and probabilistic reachable set.

\question{Why do we see the reachset violating the bounds of probabilistic
flowpipe?}
\answer{The reviewer is correct in that our choice of visualizing the
reachset or the flowpipe makes the results look incorrect. The ``ground truth
flowpipe'' in the figures is a distribution over the space of  $3\times10^5$
randomly sampled trajectories. Our previous choice of a solid color to shade the ground truth flowpipe
made it appear like a uniform distribution, which it is not. We have changed
the ground truth flowpipes to appear shaded according to the density of
trajectories. The edges of this flowpipe still indicate the
maximum and minimum value of the state components from these sampled
trajectories. Our computed $\Delta$-confident flowpipe is guaranteed to cover
 a pre-specified percentage of the trajectories, and hence some ground truth
trajectories will lie outside the $\Delta$-confident flowpipe.}

% In addition, the entrance of the bounds inside the shaded area is a promising sign that signals the accuracy of our reachability analysis. The shaded area does not represent the density of the trajectories and in fact, the portion that is outside is super sparse. The numerical examination in table 1 is also provided to show this numerically. In the new version of the figures we kept the bounds of the shaded area but we re-plotted the shaded area using color coding to show both the reachable area and the density of the trajectories inside.}\\  

\question{References regarding the christoffel function?}
\answer{Thanks for the suggestion, we have added a  comparison.}

\mypara{Reviewer 2}

\question{Explain and compare with \cite{devonport2021data} and \cite{tebjou2023data} in detail.}
\answer{We have added more explanation to the paper. 
We now briefly explain how these approaches contrast with ours. Let $v_d(x)$
denote the vector of monomials of degree up to $d$. Then, the moment matrix $M$
of a measure $\mu$ is defined as the expected value of $v_d(x)^\top v_d(x)$, and
an empirical inverse Christoffel function $\Lambda^{-1}(x)$ is defined as
$v_d(x)^\top M^{-1} v_d(x)$. The main idea in
\cite{devonport2020data,tebjou2023data} is to (empirically) determine the
sublevel set of $\Lambda^{-1}(x)$ and give probabilistic bounds on the volume of
the actual reachset that is contained in this sublevel set. The approach in
\cite{tebjou2023data} uses conformal prediction to give more accurate
probabilistic bounds on the reachset using a calibration set. There are a few
main differences between these approaches and ours: (1) The degree of the
monomials $d$ is a hyper-parameter that needs to be picked carefully (as shown
in \cite{tebjou2023data}) to avoid conservatism in the results. (2) The quality
of the results depends on how well the empirical moment matrix $M$ is estimated
from the data. (3) The dimensions of the empirical moment matrix depend on the
size of $v_d(x)$; for a system with $n$ state variables, the size of $v_d(x)$
increases exponentially in both $n$ and $d$. Given that this approach requires
inverting $M$ (an operation that is cubic in the size of $M$), with increasing
values of $d$ and $n$, this method faces scalability challenges. 
In summary, the use of Christoffel functions allows these papers to
leverage powerful results from approximation theory to estimate the number of
samples required to give probabilistic bounds on computed reachsets; however,
these methods face scalability challenges with increasing number of dimensions.}
 

% Regarding these papers,
% in our opinion, a Christoffel function also serves the role of a surrogate model, where 
% the trainable parameters are the shape matrix of the ellipsoid used in the function. The
% main approach is to separate the reachable and unreachable states using an ellipsoid in
% a much higher dimension than the dimension of the original system. The method in 
% \cite{devonport2020data} requires inverting the shape matrix, which can be cubic in the
% size of the higher-dimensional space

% However, in order to make the dataset ellipsoidally classifiable, they require increasing the dimension of the dataset noticeably, which can provide significant issues in terms of efficiency. The method proposed in \cite{devonport2021data} suffers from the inverse computation for the shape matrix, which can become prohibitively difficult if they increase the dimension of the dataset noticeably, resulting in a high-dimensional shape matrix. However, we admit, in case they can invert the shape matrix then they can cover very long horizon traces. The mentioned issue with inverse computation, implies they can not handle highly nonlinear systems and also high dimensional models, as both result in very large shape matrix for christoffel function. The surrogate model they utilize is the christofell function to learn the dataset, while we utilize Deep Neural Networks for that purpose. In our opinion, DNN is a more powerful tool than christofell function, in terms of accuracy, scalability and also the efficiency. We included a summary of this answer in the related works, where we introduce \cite{devonport2021data}. The authors in \cite{tebjou2023data} improved \cite{devonport2021data} by including conformal inference but in this work we incorporate robust conformal inference which also take care of distribution shift} \\


\question{Reach sets for higher sampling frequencies and a reasonable operating horizon for quadcopter?}
\answer{We thank the reviewer for their question and acknowledge a scalability limitation w.r.t. realistic control
frequencies in attitude control. We argue that typically we would want to
verify safety at a lower frequency (closer to the theoretical lower bound on the
frequency that maintains controllability of the system). Once this is
verified, the control frequency can be increased and the results should still
hold. Furthermore, we used a sampling time of $0.1$sec ($10$ Hz) for $50$ time
steps ($5$ sec) which was inspired by the literature on MPC for quadcopters\footnote{\url{https://www.mathworks.com/help/mpc/ug/control-of-quadrotor-using-nonlinear-model-predictive-control.html}}.
From the perspective of empirical benchmarking, we performed a new experiment
with a control frequency of $0.05$ sec ($20$ Hz) and increased our horizon to
$100$ time steps ($5$ sec). We present the new results in the revision.}

%\textcolor{red}{See Jyo's notes (make argument that we will not be able to verify at those frequency. We argue that we want to verify at a lower yet realistic time scale. Nonetheless, we performed experiments at $0.04$ seconds.  } The sampling time for the quadrotor experiment is $0.1$ seconds. This implies, for the mentioned $1$ KHz sampling frequency, our flowpipe targets one every 100 samples that you will sample, which implies reachability analysis for $5$ seconds. By the way, we also performed another experiment that performs reachability for $500$ time steps ($100$ seconds). Our experimental result shows the runtime for training has been increased noticeably, but the runtime for reachability analysis did not increase significantly. In addition, we also refer you to our response to the comment, "Examperiment, comment 8" provided for Reviewer 2.

% \question{Improve the presentation of results in the evaluation section.}\\
% \answer{We have applied your suggestions and improved presentation in the the
% evaluation section.}\\

\question{How deep is the model, and does depth matter?}
\answer{We draw the reviewers' attention to the DNN structures in the
experimental results. The model sizes range from 2 to 3 hidden layers, the
output size is always equal to $nK$ (number of dimensions times the number of
time-steps). We pick increasing number of neurons per hidden layer as it seems
to heuristically give good results. We pick a small number of hiden layers to
avoid overfitting and keep the Lipschitz constant bounded. We have not 
experimented with the hyperparameters controlling the DNN structure, though
that would be an interesting aspect to study in the future.}


% for quadrotor are all with structure $[12, 20, 400, 600]$ that is a $2$ hidden
% layer ReLU NN. and the models for Van Der Pol are all $[2,50,90, 100]$ that is
% again a $2$-hidden layer ReLU NN. There is a trade-off between the depth of the
% model and convenience for reachability. By increasing the depth the accuracy of
% the model increases but training that model is more difficult and also
% reachability on that model is more conservative. In addition, a deep model can
% result in overfitting which means unpredictable behavior on unseen data points
% which implies a high Lipschitz constant that can result in trivial bounds after
% reachability. Therefore, we are interested in a simple model to avoid
% overfitting.}\\
% 

\question{Different activation functions?}
\answer{Our proposed method applies
broadly to DNNs with arbitrary activation functions. However, as we use the NNV tool to perform efficient reachset 
computation, we focus on  ReLU
activation functions. With general activation
functions, we can use other reachset 
computation frameworks like alpha-beta-crown\footnote{``Beta-crown: Efficient bound propagation with per-neuron split constraints for neural network robustness verification'' by Wang et. al.}; however, we defer this study to future work.}




% So true. As you mentioned, some datasets are better to be trained with other activation functions. Our methodology does not require any change if the activation function is something other than ReLU and our guarantees still holds. However, in those cases we expect a higher level of conservatism as the reachability over surrogate model can be conservative.}\\  
% 
\question{Are conformal inference and prediction interchangeable?}
\answer{The terms conformal inference and conformal prediction are
interchangeable. To avoid ambiguity, we replaced conformal prediction
with conformal inference for uniformity.}

\question{For $\bar{\epsilon}$ to be valid it must be $\bar{\epsilon} > \tau$.}
\answer{You are correct. We address this aspect in Example 1.}

\question{The terms $\delta$ in $\delta$-confident flowpipe and
$\delta$-quantile are not the same.}
\answer{Yes, thanks for pointing this out. The term $\delta$ in
$\delta$-confident reachset refers to $1-\epsilon$, where $\epsilon$ is the
failure probability. So the correct notation is to use $\bar{\delta}$ to denote
$1-\bar{\epsilon}$, where $\bar{\epsilon}$ is the adjusted miscoverage level
 proposed in equation \eqref{eq:linearrule}. We have replaced $\delta$-quantile
 with $\bar{\delta}$-quantile.}

\question{Surrogate flowpipe vs. Robust flowpipe}
\answer{We call the flowpipe containing traces from the deployment environment
with confidence level of $\delta$ as the robust flowpipe. The surrogate flowpipe
is the result of deterministic reachability on surrogate model, which is denoted
$\bar{X}$. We note that the robust flowpipe is derived from the surrogate
flowpipe using robust conformal inference.}

\question{What if distribution shift exceeds threshold
$\tau$?}
\answer{If the actual distribution shift is more than the radius
$\tau$, then we cannot give any guarantees using robust conformal inference.
However, from \cite[Corollary 2.1]{cauchois2020robust} we see that the guarantees degrade smoothly if the distribution shift is beyond $\tau$. In our experiments, we picked $\tau$ to be more than the estimated distribution shift in the
residual space (induced by the distribution shift in the model parameter
space).} 

% \answer{Thanks, the extent of violation in the scenario that you proposed is entirely dependent on the distribution of deployment environment. We utilize Total-variation to show the distribution shift. Consider the deployment environments $b$ and $c$ that have similar distribution shift to training environment $a$. In this case, the distribution of $b$ and $c$ can be significantly different. For example, an increase in distribution for $b$ may still keep our guarantee, while for $c$, that may violate it noticeably. }\\


\question{Is $\tau = 0$ a valid scenario in robust conformal inference? }
\answer{The expression $\tau > 0$ was an unfortunate typo, it should read $\tau \ge 0$. The 
case when $\tau = 0$ is the case when there is no distribution shift, which is effectively
addressed by vanilla conformal inference.}

\question{Missing axis labels, Concerns about the figure, Missing description for quadcopter states}
\answer{We have overhauled the figures to add clarity, and added details about
the states of the quadcopter.}

\question{Reachability between time $40$ to $90$?} \answer{We apologize if the
reviewer understood our flowpipe construction as being repeated at every
time-step. This is certainly a good idea that we can consider in the future,
where we repeat flowpipe computation in a receding horizon fashion. In the
current paper, this is {\bf not} our objective, we are only looking at the
problem of computing the flowpipe over the first $\horizon$ steps (at sampling-time $\delta t$). To
implement such ``online and receding horizon'' style flowpipe computation, one
technical detail that will need to be addressed is that to compute the flowpipe
starting from an arbitrary time $k$, the set of initial states is the set of
states reachable at time $k$; this set has an unknown distribution. But we
can sample from this distribution by considering simulated $k$-long trajectories (starting from time $0$ and ending in time-step $\timeid$), but this does not scale with increasing $k$ as the simulation from time $0$ can be time consuming.}


% In case we are in step $40$ and want to perform reachability analysis for steps, $41-90$ we can not utilize the previous surrogate model that is trained for steps $1-50$. This is because we utilize the traces that start from initial states and propagate up to $50^{\text{th}}$ time step, to train our model. We suggest following these steps to perform the reachability. 1) Perform our reachability analysis with confidence $\delta_1$ for the flowpipe $X_{0-40}$ spanning over $0\leq \timeid \leq 40$. 2) Extract the reachset for $\timeid =40$, $\init_{40}$, from the flowpipe $X_{0-40}$ that is in fact a $\delta_1$-confident polytope. 3) Train a new model that receives $s_{40} \in \init_{40}$ and predicts $s_{41}, \ldots, s_{90}$. 4) Perform our reachability analysis with confidence $\delta_2$ for the flowpipe $X_{40-90}$ spanning over $40\leq \timeid \leq 90$. 5) Utilize union bound and compute the overall level of confidence for the flowpipe $X_{40-90}$, that is $\delta = 1- (2- \delta_1 -\delta_2)$. }

\mypara{Reviewer 3}

\question{Reliability of the result, and concerns about upper bound on distribution shift.}
\answer{We agree that assuming knowledge of an upper bound on the distribution
shift $\tau$ is a non-trivial assumption. However, we note that similar assumptions are standard in other communities, e.g., in robust control   where upper
bounds on the difference between the real system and the system model are routinely assumed. The same argument holds
here, e.g., it is better to have robustness than not having robustness. Note that robust reachability analysis will generally be impossible to perform without
assuming such an upper bound. We also remark that this is a
standard assumption in the field of robust conformal inference. We further note
that the user {\em can} estimate an upper bound on the distribution shift using
sampling-based techniques, see \cite{zhao2023robust,cauchois2020robust} 
for examples. Regarding the accuracy and fidelity of the surrogate model, we emphasize that
the main role of conformal inference is to systematically perform error
analysis, and hence model accuracy and fidelity is precisely what our methods
can quantify via calibration.}
%We clarified in the document that the distribution shift here is upper bounded with a user-specified parameter. In case no upper bound on distribution shift is known, then the concept of reachability will be totally meaningless, as we don't even know whether deployment environment is related to training environment or not. The user can come up with an upper bound empirically via sampling or many other techniques. In our opinion, if the reader has concern about the imprecision of the model, that implies he/she is rejecting the idea of combining AI and reachability. This is because the imprecision is a well-known problem in machine learning, and others use accuracy and error analysis to monitor it. In case the model is not precise enough, it is routine to train it again. This paper is all about probabilistic guarantee, and we were able to provide it by combining AI and reachability. Regarding the concern about use-case of reachability, we can list: verification, monitoring and abstraction based control synthesis. Regarding the concern about the reliability of conclusion, we provided the toolbox online which can be used for repeatability evaluation.}\\

\question{Concern about novelty and technical contribution} \answer{We emphasize that our work is the first to address 
the sim2real gap in formal reachability analysis, and the first
to propose efficient robust reachability tools to solve a practically motivated problem. Previous work in
\cite{hashemi2023data,devonport2021data,tebjou2023data} consider the problem of
data-driven reachability analysis, but do not consider the possibility of
distribution shifts. Compared to the work in \cite{hashemi2023data}, we also consider
training with a quantile loss, using optimization to bound the area of the
flowpipe, and reducing conservatism induced by multi-dimensional and
multi-time-step probabilistic guarantees. 

We humbly disagree with the reviewer that our method is just a combination of different techniques,
because to address reachability of real-world systems, we have combined
components in a novel way using techniques from optimization and statistical
learning: (1) a na\"{i}ve combination with \cite{hashemi2023data} would just add reasoning
about distribution shifts, but would suffer from extensive conservatism due to union
bounding over multi-time-step and multi-dimensional prediction errors, (2) the use of MSE-based loss as in \cite{hashemi2023data} will
result in heavy tailed distributions as opposed to the quantile loss (see 
Experiment 1), and (3) we get significant improvement in data efficiency by utilizing the residual proposed in \cite{cleaveland2023conformal} while minimizing for the volume of the flowpipe 
 (see Experiment 2).}

\question{Role of calibration dataset $\calibdataset$} 
\answer{Conformal inference
is a technique to provide probabilistic guarantees 
for predictions made by surrogate models. Importantly, conformal inference does this independently of the quality of the trained model and for arbitrary surrogate models (e.g., feedforward or recurrent NNs). Conformal inference works as follows:
(1) We train a predictor (in our case a $K$-step trajectory is predicted from
the initial state) using some training data (in our case sampled initial states and trajectories from  simulation). (2)
We sample i.i.d. data from the same distribution (i.e.  initial states and
trajectories), then we use the loss function to define a non-conformity score.
The set of non-conformity scores is $\calibdataset$. (3) Then this set is sorted,
and the $\lceil(m+1)(1-\epsilon)\rceil^{th}$ quantity from this set is computed
(denoted $R^*_{1-\epsilon}$). Conformal inference guarantees that the residual
error for a prediction from {\em any previously unseen state} has to be less
than $R^*_{1-\epsilon}$ with probability greater than $1-\epsilon$.  This is
discussed in Section~\ref{sec:prelim} under ``Conformal Inference.'' Thus, the
calibration set can help us reason about the accuracy and fidelity of the model,
using results from statistical learning.}

% The accuracy of the model impacts the tightness of the flowpipe but it doesn't impact the validity of the proposed guarantee. In other words, an inaccurate model will result in a conservative and large flowpipe but even for that conservative flowpipe the probabilistic guarantee still holds. The mentioned argument is supported with the theory of conformal inference. In fact conformal inference, takes care of statistical analysis of model's error no matter how inaccurate it is. The calibration dataset is utilized for error analysis via conformal inference and once the model is trained from training dataset we generate our probabilistic guarantee based on calibration dataset. In the paper, we proposed a zonotope called inflating zonotope and we claim in case we inflate the reach set of surrogate model with this zonotope then the resulting flowpipe offers the probabilistic guarantee in the real world. In fact, we generate the inflating zonotope from error analysis of the model over the calibration dataset. Based on the rules of conformal inference, we are not allowed to use training dataset for error analysis via conformal inference. We have also included the distribution of residual errors after the training process to the revised document. This is added to evaluate the quality of the model.}\\

\mypara{Reviewer 4}

\question{Parameter $R_i$ is used before it is introduced}
\answer{Thank you for spotting this. We have accounted for it.}

\question{Perform a comparison with related research.}
\answer{There are two bodies of work that we could potentially compare against,
but the comparisons would either not be apples-to-apples or would be unfair. The
works in \cite{devonport2021data, tebjou2023data} do not compute flowpipes and
instead compute a single reachset containing all trajectory points, making a
like-for-like comparison difficult. Furthermore, the results in
\cite{tebjou2023data} vary based on the specific hyper-parameters of the
Christoffel functions, which would necessitate tuning these for our examples.
Finally, we note that the number of monomials for a 12-dimensional system (such
as the quadcopter example we consider) with degree up to $4$ is ${12+4 \choose
4} = 1820$, which means that the shape matrix is of size $1820\times 1820$.
Obtaining such a large matrix empirically would need very large amounts of data.
There are several model-based reachability techniques that exist, but a
comparison against them would be unfair as these assume knowledge of the
dynamics in a symbolic form.}

\noindent {\bf Summary.} Edits in the revision are shown in blue. The main
changes are: a) related work moved to the beginning, b) more explanation added
to compare against related work, c) added details about surrogate models and
design choices,  d) included a new quadrotor experiment to address R2's comment
about the sampling time, e) improved the clarity of all the figures, f) added a
new figure showing the distribution of residual errors after training to
illustrate the quality of the surrogate model.

